SoK: Memorisation in machine learning

Quantifying the impact of individual data samples on machine learning models is an open research problem. This is particularly relevant when complex and high-dimensional relationships have to be learned from a limited sample of the data generating distribution, such as in deep learning. It was previously shown that, in these cases, models rely not only on extracting patterns which are helpful for generalisation, but also seem to be required to incorporate some of the training data more or less as is, in a process often termed memorisation. This raises the question: if some memorisation is a requirement for effective learning, what are its privacy implications? In this work we unify a broad range of previous definitions and perspectives on memorisation in ML, discuss their interplay with model generalisation and their implications of these phenomena on data privacy. Moreover, we systematise methods allowing practitioners to detect the occurrence of memorisation or quantify it and contextualise our findings in a broad range of ML learning settings. Finally, we discuss memorisation in the context of privacy attacks, differential privacy (DP) and adversarial actors.

==> influence_old.tex <==
\section{Measuring memorisation by estimating influence}
As per \ref{sec:feldman}, memorisation can be measured directly using the concepts of \textit{influence} (and in particular \textit{self-influence}).
In this section, we discuss influence in detail and outline how it can be quantified.
It is of note that in this work we refer to \textit{self-influence} as \textit{influence} (in contrast to \textit{cross-influence}), unless specified otherwise.

The influence of individual samples is canonically estimated through a \say{leave-one-out} (LOO) re-training technique (i.e. how much does performance change when a single sample is removed) \cite{cook1977detection}.
However, this results in a requirement to train at least as many models as there are points in the dataset.
Moreover, since neural networks are typically non-deterministic with respect to initialisation and other hyperparameters, potentially several copies of each network have to be trained, resulting in a computationally untenable situation.
Therefore, a number of suitable \textit{estimators} of sample influence have previously been proposed, mainly concentrating on the concept of influence functions \cite{koh2017understanding}.

The direct computation of influence functions has specific computational constraints (notably the requirement for second-order derivatives), \cite{feldman2020neural} utilise a \textit{Monte Carlo} technique to compute the expected memorisation of $y_i$ on a random subset of $S$ that includes $m\le n$ samples. 
This approximation has a number of traits: it can be seen as a $mem(A, S, i)$ smoothed by random subsampling; it can be estimated with standard deviation of $\sigma$ for every $i$ at the same time using $O(1/\sigma^2)$ runs and it also closely related to the concept of the Shapley value \cite{ghorbani2019data} (which we discuss in detail below) of sample $i$ with respect to its self-accuracy.

\subsection{Influence function estimation}
\label{sec:influence}
There exists a number of methods which can be used to estimate the influence of individual samples.
A recent paper by \cite{hammoudeh2022training} discusses influence estimation in detail, and we refer to this work for details on the various techniques.
Here, we outline a subset of these approaches to influence estimation, focusing on the direct computation or the computation of efficient proxies for the influence function value.
Influence functions attempt to approximate the effect of LOO re-training without necessitating additional training runs.
The seminal work of \cite{koh2017understanding} ported the notion of \textit{influence functions} from the domain of robust statistics to deep learning. 
Similar to their utilisation in statistics, the aforementioned paper proposes the utilisation of second-order derivatives (i.e. the Hessian matrix) to compute the influence function values.
Intuitively, through a second-order Taylor series expansion, the effect of a small perturbation (which is assumed to be induced by the removal of a single sample similar to LOO re-training) on the loss function can be approximated.
Evidently, Hessian matrices are infeasible to compute for large neural networks, requiring memory which is squared in the number of network parameters.
Specific techniques for efficient estimation of second-order derivative-based influence functions have been proposed to tackle this issue \cite{guo2020fastif, schioppa2022scaling}, allowing for the utilisation of influence functions even in models as large as recent-generation large language models \cite{grosse2023studying}.
We note that the exact semantics of influence functions (at least in terms of cross-influence) are still a topic of active investigation \cite{schioppa2023theoretical, bae2022if}.
An alternative approach relies on using the so-called \say{representer theorem}, allowing the model owner to decompose the prediction into individual contributions (i.e. influences) from each data instance \cite{yeh2018representer}.
This method was originally proposed for linear models but has later been extended to neural networks \cite{chen2021hydra}.

Nonetheless, the more or less direct computation of influence function values remains computationally cumbersome.
We note that, although related in terms of their utilisation of second-order derivatives, techniques which estimate the curvature of the loss function with respect to individual inputs (instead of weights) are distinct from influence function estimation techniques, but have also been used to measure memorisation \cite{katharopoulos2018not, garg2023memorization}.
Moreover, techniques attempting to derive a proxy for the influence function value while not requiring second-order derivatives have been developed, such as techniques which \textit{trace} the evolution of the loss function's value or the (first order) gradient through training have been proposed \cite{pruthi2020estimating, hammoudeh2022identifying}.
Moreover, distinct techniques to estimate training data influence or memorisation utilising \textit{only} first-order gradient quantities are of significant interest, as these quantities can be very efficiently computed in current deep learning frameworks.

\begin{tcolorbox}[colback=gray!10!white, colframe=white!50!black, title=Key Point]
  Influence is impossible to calculate directly using second-order derivatives, so approximations have to be used.
\end{tcolorbox}

\subsection{Data valuation}
\label{sec:valuation}
In this section, we discuss the relationship between the study of memorisation and the study of data \textit{valuation}.
The connection between the two concepts is salient, seeing as samples which are of high value to the model (that is, they improve the model's performance the most), are often also samples which are highly influential.
This in turn, means that they are also often highly memorised.
We note that valuation is a complex and multi-faceted topic and refer to the survey \cite{ni2020survey} for a detailed overview.
Moreover, it is important to bear in mind that the concept of \textit{value} should ideally be expressed in relation to a pre-determined standard, such as the accuracy increase on a pre-defined, unseen dataset which is agreed upon between parties, linking it to (out-of-sample) generalisation.
As such, this concept is conceptually close to a notion of cross-influence where any given sample can either have a beneficial effect on generalisation (=high value) or no beneficial effect (=low value).
In comparison, the canonical notion of cross-influence also considers the possibility of negative influence, i.e. a sample being harmful to generalisation. 
Such a notion can only be expressed in valuation frameworks which allow for negative valuation scores.
As discussed above, atypical samples are often associated with high memorisation.
This reveals that the concept of memorisation is --in a sense-- orthogonal to valuation: a sample can be highly memorised without actually having high value to the model and vice versa (as we demonstrate on Figure \ref{fig:influence_map}).
Nonetheless, the concepts are often used synonymously in the sense that methods which in reality measure sample difficulty, influence or a lack of typicality, are presented as measuring sample value.
These include many of the aforementioned, such as loss values, gradient magnitudes, etc. \cite{goetz2019active, lai2021oort, salehi2018coordinate, shah2020choosing, lee2020accurate}.
While these metrics are popular in literature across a variety of learning settings \cite{cho2022towards, tang2022fedcor, ren2018learning, fan2022improving, goetz2019active}, their lack of robustness hinders their interpretability and utilisation as proper memorisation metrics (for example, loss values tend be lower in later training rounds \cite{shin2022fedbalancer, lai2021oort}).
Moreover, these values lack an axiomatic interpretation in the sense that they do not measure the \say{independent} value of individual samples, but are highly correlated among samples (thus, even a different sample ordering would change the score).
This is in contrast with formal measures of data value, which we discuss next.

\textbf{Game-theoretic approaches}
In collaborative ML, particularly in federated learning, methods which allow a federation of clients to compute the value of their data without sharing it has recently been popularised \cite{kwon2021beta, merrick2020explanation, ghorbani2019data}. 
In particular, as these learning settings represent a collaborative \say{game}, where the federation is trying to maximise model performance while minimising the computation cost, approaches based on concepts from game theory have been widely used \cite{wang2019measure, sim2020collaborative, wang2023data}.

Arguably, the most significant game-theoretic valuation metric is the Shapley value, whose definition is derived axiomatically and thus satisfies a number of desirable characteristics.
Its use was extended to data valuation by \cite{ghorbani2019data} to express the expected marginal contribution of individual data points.
Shapley values are truly marginal contribution scores, i.e. are computed with respect to \textit{all possible} subsets (coalitions) a data point could be part of, contrary to many of the aforementioned techniques.
Among other useful properties, all marginal contributions sum to the contribution of the entire dataset (efficiency) and individual contributions are additive.
Moreover, contributions of \textit{useless} data points are zero.
Due to these beneficial characteristics, Shapley values have been widely adopted in a number of works on data valuation and, in particular, in distributed settings \cite{jiang2023fair, ling2022fedentropy, ghorbani2019data}.
A conceptually similar value to the Shapley value is the Banzhaf value, which has also been utilised for data valuation \cite{wang2023data}. 
Banzhaf values are similar to Shapley values, but satisfy additional robustness properties.
This is beneficial, as game-theoretic valuation measures can suffer from a lack of robustness to re-initialisation of the model \cite{kwon2021beta}, requiring averaging over several model initialisations.
This is however problematic, as the computation of Shapley and Banzhaf values requires computing the contribution of a data sample over \textit{all possible} combinations, resulting in exponential time complexity, which is infeasible for all but the fastest-training models.
Although Shapley and Banzhaf values are not direct measures of memorisation, their definition shares similarities with the influence score proposed by \cite{feldman2020neural} and, as such, have been used as proxies of memorisation \cite{bloch2021data}.

\begin{tcolorbox}[colback=gray!10!white, colframe=white!50!black, title=Key Point]
  Game-theoretic approaches can be used to identify samples of high influence, which are often more prone to memorisation 
\end{tcolorbox}
